Markov Stochastic Choice

We examine the effect of item arrangement on choices using a novel decision-making model based on the Markovian exploration of choice sets. This model is inspired by experimental evidence suggesting that the decision-making process involves sequential search through rapid stochastic pairwise comparisons. Our findings show that decision-makers following a reversible process are unaffected by item rearrangements, and further demonstrate that this property can be inferred from their choice behavior. Additionally, we provide a characterization of the class of Markovian models in which the agent makes all possible pairwise comparisons with positive probability. The intersection of reversible models and those allowing all pairwise comparisons is observationally equivalent to the well-known Luce model. Finally, we characterize the class of Markovian models for which the initial fixation does not impact the final choice and show that choice data reveals the existence and composition of consideration sets.

==> input/figure/fig-model4.tex <==
	\begin{tikzpicture}[->,shorten >=1pt,auto,node distance=4cm, scale=0.5]
		\begin{scope}[every node/.style={circle,draw,minimum size=0.7cm}]
		    \node (i) at (0,0) {$i$};
		    \node[fill=corallight] (j) at (2.5,0) {$j$};
		    \node (l) at (0,2.5) {$l$};
		    \node (k) at (2.5,2.5) {$k$};
		\end{scope}
	\end{tikzpicture}

==> input/text/app-3-proof-T2-cor.tex <==
\subsection{Proof of Corollary~\ref{cor:T2-positive}}
\label{proof:T2-cor}
\textbf{(a) $\implies$ (b):} If the \msc[l] is fully comparable, Theorem~\ref{T2} implies that the generated stochastic choice function is such that for all pairs $i,j\in\M$ with $\del[ij]{\M}\neq 0$, $\exists \cyr[]{\M'}{\M}$ with $(i,j)\in\cyr[]{\M'}{\M}$. The positivity of the stochastic choice function follows directly from the Perron–Frobenius theorem.


\textbf{(b) $\implies$ (a):} We know from Theorem~\ref{T2} that if a stochastic choice function is such that for all pairs $i,j\in\M$ with $\del[ij]{\M}\neq 0$, $\exists \cyr[]{\M'}{\M}$ with $(i,j)\in\cyr[]{\M'}{\M}$, it is rationalizable by a pairwise comparable \msc[l]. Consider the construction of the rationalizing model given in the proof of the theorem in Appendix~\ref{proof:T2}. Since ${\sav{}\gg \boldsymbol{0}}$, it holds for all $(i,j)\in\G$ that $\q{ij}{\M}>0$. It is easy to see that the positivity of the stochastic choice function ensures that all other transition probabilities are positive as well, hence the constructed model is fully comparable.

\textbf{(b) $\implies$ (c):} Consider a positive stochastic choice function $\bp[\M]$ and a pair $(i,j)\in\M$ with $\del[ij]{\M}\neq 0$ such that $\exists \cyr[]{\M'}{\M}$ with $(i,j)\in\cyr[]{\M'}{\M}$. Assume without loss of generality that $(i,j)\in\cyr[-]{\M'}{\M}$. Then, it holds for all $(k,l)\in\cyr[-]{\M'}{\M}$ that
$$\frac{\p{k}{\M}}{\p{l}{\M}}<\frac{\p{k}{\set{k,l}}}{\p{l}{\set{k,l}}}.$$


==> input/text/app-4-proof-time-pressure.tex <==
\subsection{Proof of Proposition~\ref{prop:time-pressure}}
\label{proof:time-pressure}
Fix a menu $\M\in\Nset$ and let $\bra[]{\delta_i}{\mat[]{\M}}$ denote the stochastic choice function generated by the \msc[b] with initial distribution equal to the degenerate distribution with point mass on alternative~$i$. 
	We will first show that a stochastic choice function is a linear combination of the stochastic choice functions from degenerate initial conditions. Let ${V=(I-(1-\abs)\mat[]{\M})}$ and ${W=V^{-1}}$, which exists for $\abs \neq 0$. Recall from equation~\eqref{eq-def} that
	\begin{align*}
	\bra[]{\init[]{}}{\mat[]{\M}}&= \abs \init{}{} (I-(1-\abs)\mat[]{\M})^{-1}=\abs \init{}{}V^{-1}=\abs \init{}{}W. 	
	\end{align*}
Since we have fixed $\abs$ and $\mat[]{\M}$ we will use the following simplified notation to denote the probability to choose alternative $i$ from the menu $\bra[i]{\init[]{}}{\mat[]{\M}}=\rode{i}{\boldsymbol{\pi}}$. 

Note that $\rode{i}{\delta_j}=\abs w_{ji}$ for any $i,j\in \M$. If $\init{}{}$ is not degenerate, we have that 
\begin{equation}
\label{deg-sum}
\rode{i}{\boldsymbol{\pi}}=\sum_{j\in \M}\init[j]{}\abs w_{ji}=\sum_{j\in \M}\init[j]{} \rode{i}{\delta_j}\quad \forall i\in\M.
\end{equation}
	Let $i$ be the target alternative. We will now show that ${\rode{i}{\delta_i}> \rode{i}{\delta_j}}$ for all $j\neq i$. Denote ${\max_{j\neq i}\{\rode{i}{\delta_j}\}=\rode{i}{\delta_m}}$. Since $V\cdot W=I$ we obtain the following equation when we multiply $V$'s $m^\text{th}$ row vector with $W$'s $i^\text{th}$ column vector:
	\begin{equation*}
	\begin{gathered}
		(1-(1-\abs)\q{mm}{})w_{mi}+\sum_{j \neq m}(-1)(1-\abs)\q{mj}{}w_{ji}=0\\
	(1-(1-\abs)(1-\sum_{j\neq m}\q{mj}{}))w_{mi}-(1-\abs)\sum_{j \neq m}\q{mj}{}w_{ji}=0\\
		(\abs+(1-\abs)\sum_{j\neq m}\q{mj}{})w_{mi}-(1-\abs)\sum_{j \neq m}\q{mj}{}w_{ji}=0\\
		(1-\abs)(\sum_{j\neq m}\q{mj}{}(w_{ji}-w_{mi}))=\abs w_{mi}
				\end{gathered}
	\end{equation*}
Finally, we plug in $\rode{i}{\delta_j}=\abs w_{ji}$ and obtain
	\begin{equation*}
	\begin{gathered}
		\sum_{j\neq m}\q{mj}{}(\rode{i}{\delta_j}-\rode{i}{\delta_m})=\frac{\abs}{1-\abs} \rode{i}{\delta_m}.
		\end{gathered}
	\end{equation*}
We assumed w.l.o.g.\ that $\rode{i}{\delta_m}\geq \rode{i}{\delta_j}$ for all $j\neq i$. If $\rode{i}{\delta_m}\geq \rode{i}{\delta_i}$, then the left-hand side of the above equation is weakly negative, which is a contradiction. Therefore, $\rode{i}{\delta_i}> \rode{i}{\delta_j}$ for all $j\neq i$. Consider now the difference in the choice probability of $i$ using equation~\eqref{deg-sum} and that ${\sum_{j}\Delta\init[j]{}=0}$:
\begin{equation*}
\begin{aligned}
\rode{i}{\boldsymbol{\pi}'}-\rode{i}{\boldsymbol{\pi}}&=\Delta\init[i]{}\rode{i}{\delta_i}+\sum_{j\neq i}\Delta\init[j]{}\rode{i}{\delta_j}\\
&=-\sum_{j\neq i}\Delta\init[j]{}\rode{i}{\delta_i}+\sum_{j\neq i}\Delta\init[j]{}\rode{i}{\delta_j}\\
&=\sum_{j\neq i}\Delta\init[j]{}(\rode{i}{\delta_j}-\rode{i}{\delta_i})> 0,
\end{aligned}
\end{equation*}	
where the last inequality follows from the assumption that $\Delta\init[j]{}\leq 0$ for all $j\neq i$.

==> input/text/app-5-proof-metro.tex <==
\subsection{Proof of Corollary~\ref{cor:metro}}
\label{proof:metropolis}
We show that among the rationalizing models there is always going to be a model with symmetric relative salience parameters by letting $\tr{ij}=\p[c]{j}{i,j}$ for all $i,j\in\all$. We then generate the rationalizing \msc[l] from choice data analogously as shown in the proof of Theorem~\ref{T1}. If $\q{ij}{}=\q{ji}{}=0$, then $\sa{ij}{}=\sa{ji}{}=0$. Having $\q{ij}{}>0$ and $\q{ji}{}=0$ implies $\q[c]{ji}{i,j}=0$ and $\tr{ji}=0$. We can then let $\sa{ji}{}=\sa{ij}{}$. Finally, if $\q{ij}{}>0$ and $\q{ji}{}>0$, TR-IIA implies that $\sa{ji}{}=\sa{ij}{}\frac{\tr{ij}}{\tr{ji}}\frac{\p[c]{i}{i,j}}{\p[c]{j}{i,j}}=\sa{ij}{}$. Therefore, the constructed model rationalizes the choice data and has symmetric relative salience parameters.
